Stellar magnetosphere reconstruction from radio data. Multi-frequency VLA observations and 3D-simulations of CU Virginis

In order to fully understand the physical processes in the magnetospheres of the Magnetic Chemically Peculiar stars, we performed multi-frequency radio observations of CU Virginis. The radio emission of this kind of stars arises from the interaction between energetic electrons and magnetic field. The radio data were acquired with the VLA and cover the whole rotational period of CU Virginis. For each observed frequency the radio light curves of the total flux density and fraction of circular polarization were fitted using a three-dimensional MCP magnetospheric model simulating the stellar radio emission as a function of the magnetospheric physical parameters. The observations show a clear correlation between the radio emission and the orientation of the magnetosphere of this oblique rotator. Radio emission is explained as the result of the acceleration of the wind particles in the current sheets just beyond the Alfv\'en radius, that eventually return toward the star following the magnetic field and emitting radiation by gyrosyncrotron mechanism. The accelerated electrons have a hard energetic spectrum ($N(E)\propto E^{-2}$) and the acceleration process has an efficiency of about $10^{-3}$. The Alfv\'en radius we determined is in the range of $12-17 R_\ast$ and, for a dipolar field of 3000 Gauss at the magnetic pole of the star, we determine a mass loss from the star of about $10^{-12}$ M$_{\sun}$ yr$^{-1}$. In the inner magnetosphere a detectable X-ray emission is expected.

==> tab1.tex <==
%\documentstyle[12pt]{article}
%\pagestyle{empty}
%\textwidth 25 cm
%\textheight 28 cm
%\topmargin -2 cm
%\oddsidemargin -5cm
%\begin{document}

\footnotesize
\begin{center}
\begin{tabular}{cccrcccrccc}
\hline
\hline
 {\footnotesize $\langle$UT$\rangle$} & {\footnotesize $I_5~~(\sigma)$} 	&{\footnotesize $V_5~~(\sigma)$}	&{~~~~}
& {\footnotesize $\langle$UT$\rangle$} & {\footnotesize $I_{8.4}~~(\sigma)$}	&{\footnotesize $V_{8.4}~~(\sigma)$}	&{~~~~}
& {\footnotesize $\langle$UT$\rangle$} & {\footnotesize $I_{15}~~(\sigma)$}	&{\footnotesize $V_{15}~~(\sigma)$}	\\
 &{\scriptsize [mJy]} &{\scriptsize [mJy]} &{~~~~}
& &{\scriptsize [mJy]} &{\scriptsize [mJy]} &{~~~~}
& &{\scriptsize [mJy]} &{\scriptsize [mJy]} \\
\hline
%&&&&&&&\\
\multicolumn{11}{c}{\scriptsize Date: 1998 June 02}\\
%&&&&&&&\\
\hline
 {\scriptsize 00:30:45}  &{\scriptsize $2.78~~(0.05)$} &{\scriptsize $<3\sigma~~(0.05)$} &{~~~~}
& {\scriptsize 01:37:00}  &{\scriptsize $3.18~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 02:51:50}  &{\scriptsize $4.1~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 01:23:05}  &{\scriptsize $3.27~~(0.05)$} &{\scriptsize $~~0.32~(0.05)$} &{~~~~}
& {\scriptsize 02:36:55}  &{\scriptsize $3.87~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 03:51:35}  &{\scriptsize $4.3~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 02:22:55}  &{\scriptsize $3.64~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 03:38:50}  &{\scriptsize $4.40~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 04:51:25}  &{\scriptsize $3.4~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 03:22:45}  &{\scriptsize $4.13~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 04:36:35}  &{\scriptsize $4.42~~(0.03)$} &{\scriptsize $<3\sigma~~(0.03)$} &{~~~~}
& {\scriptsize 05:51:20}  &{\scriptsize $3.3~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 04:22:35}  &{\scriptsize $4.44~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 05:36:30}  &{\scriptsize $3.69~~(0.03)$} &{\scriptsize $<3\sigma~~(0.03)$} &{~~~~}
& {\scriptsize 06:51:15}  &{\scriptsize $2.1~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 05:22:25}  &{\scriptsize $3.48~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 06:36:20}  &{\scriptsize $2.85~~(0.03)$} &{\scriptsize $<3\sigma~~(0.03)$} &{~~~~}
& {\scriptsize 07:44:20}  &{\scriptsize $3.0~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 06:22:15}  &{\scriptsize $2.78~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 07:30:25}  &{\scriptsize $2.85~~(0.04)$} &{\scriptsize $~~0.22~(0.04)$} &{~~~~}
& {\scriptsize \dots}  &{\scriptsize \dots} &{\scriptsize \dots} 	\\
%&&&&&&&&&\\
 {\scriptsize 07:18:55}  &{\scriptsize $3.96~~(0.05)$} &{\scriptsize $~~0.58~(0.05)$} &{~~~~}
& {\scriptsize \dots}  &{\scriptsize \dots} &{\scriptsize \dots} &{~~~~}
& {\scriptsize \dots}  &{\scriptsize \dots} &{\scriptsize \dots} 	\\
%&&&&&&&&&\\
 {\scriptsize 08:13:45}  &{\scriptsize $3.57~~(0.05)$} &{\scriptsize $~~0.27~(0.05)$} &{~~~~}
& {\scriptsize \dots}  &{\scriptsize \dots} &{\scriptsize \dots} &{~~~~}
& {\scriptsize \dots}  &{\scriptsize \dots} &{\scriptsize \dots} 	\\
%&&&&&&&&&\\
\hline
%&&&&&&&\\
\multicolumn{11}{c}{\scriptsize Date: 1998 June 07}\\
%&&&&&&&\\
\hline
 {\scriptsize 02:10:15}  &{\scriptsize $4.87~~(0.04)$} &{\scriptsize $~~0.43~(0.04)$} &{~~~~}
& {\scriptsize 02:23:40}  &{\scriptsize $4.85~~(0.03)$} &{\scriptsize $~~0.77~(0.03)$} &{~~~~}
& {\scriptsize 02:38:10}  &{\scriptsize $3.3~~(0.1)$} &{\scriptsize $~0.4~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 03:08:35}  &{\scriptsize $4.87~~(0.04)$} &{\scriptsize $~~0.37~(0.04)$} &{~~~~}
& {\scriptsize 03:21:35}  &{\scriptsize $4.97~~(0.03)$} &{\scriptsize $~~0.56~(0.03)$} &{~~~~}
& {\scriptsize 03:35:55}  &{\scriptsize $3.0~~(0.1)$} &{\scriptsize $<3\sigma~(0.1)~$} 	\\
%&&&&&&&&&\\
 {\scriptsize 04:06:25}  &{\scriptsize $4.68~~(0.04)$} &{\scriptsize $~~0.34~(0.04)$} &{~~~~}
& {\scriptsize 04:19:25}  &{\scriptsize $4.52~~(0.03)$} &{\scriptsize $~~0.57~(0.03)$} &{~~~~}
& {\scriptsize 04:33:45}  &{\scriptsize $3.6~~(0.15)$} &{\scriptsize $<3\sigma~(0.15)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 05:04:50}  &{\scriptsize $3.73~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 05:18:20}  &{\scriptsize $3.50~~(0.04)$} &{\scriptsize $~~0.28~(0.04)$} 	  &{~~~~}
& {\scriptsize 05:32:45}  &{\scriptsize $3.3~~(0.15)$} &{\scriptsize $<3\sigma~(0.15)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 06:03:35}  &{\scriptsize $3.79~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 06:17:05}  &{\scriptsize $3.88~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 06:31:35}  &{\scriptsize $3.4~~(0.15)$} &{\scriptsize $<3\sigma~(0.15)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 07:02:30}  &{\scriptsize $3.98~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 07:15:15}  &{\scriptsize $4.01~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize \dots}     &{\scriptsize \dots} &{\scriptsize \dots} 	\\
%&&&&&&&&&\\
 {\scriptsize 07:54:30}  &{\scriptsize $4.38~~(0.05)$} &{\scriptsize $<3\sigma~~(0.05)$} &{~~~~}
& {\scriptsize \dots}	  &{\scriptsize \dots} 		&{\scriptsize \dots} 	  &{~~~~}
& {\scriptsize \dots}  	  &{\scriptsize \dots} 		&{\scriptsize \dots} 	\\
\hline
%&&&&&&&\\
\multicolumn{11}{c}{\scriptsize Date: 1998 June 12}\\
%&&&&&&&\\
\hline
 {\scriptsize 01:21:35}  &{\scriptsize $3.95~~(0.05)$} &{\scriptsize $<3\sigma~~(0.05)$} &{~~~~}
& {\scriptsize 01:35:05}  &{\scriptsize $4.31~~(0.04)$} &{\scriptsize $-0.14~(0.04)$} &{~~~~}
& {\scriptsize 02:47:25}  &{\scriptsize $3.3~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 02:19:55}  &{\scriptsize $4.10~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 02:32:55}  &{\scriptsize $4.18~~(0.04)$} &{\scriptsize $-0.21~(0.04)$} &{~~~~}
& {\scriptsize 03:45:15}  &{\scriptsize $2.5~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 03:17:45}  &{\scriptsize $3.47~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 03:30:45}  &{\scriptsize $3.54~~(0.03)$} &{\scriptsize $<3\sigma~~(0.03)$} &{~~~~}
& {\scriptsize 04:44:10}  &{\scriptsize $2.7~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 04:16:05}  &{\scriptsize $3.12~~(0.04)$} &{\scriptsize $<3\sigma~~(0.04)$} &{~~~~}
& {\scriptsize 04:29:35}  &{\scriptsize $3.05~~(0.03)$} &{\scriptsize $~~0.16~(0.03)$} &{~~~~}
& {\scriptsize 05:43:00}  &{\scriptsize $3.3~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 05:15:05}  &{\scriptsize $3.28~~(0.04)$} &{\scriptsize $~~0.50~(0.04)$} &{~~~~}
& {\scriptsize 05:28:25}  &{\scriptsize $3.58~~(0.03)$} &{\scriptsize $~~0.39~(0.03)$} 	  &{~~~~}
& {\scriptsize 06:41:50}  &{\scriptsize $3.7~~(0.1)$} &{\scriptsize $<3\sigma~~(0.1)$} 	\\
%&&&&&&&&&\\
 {\scriptsize 06:13:55}  &{\scriptsize $4.38~~(0.04)$} &{\scriptsize $~~0.44~(0.04)$} &{~~~~}
& {\scriptsize 06:27:20}  &{\scriptsize $4.33~~(0.03)$} &{\scriptsize $~~0.53~(0.03)$} &{~~~~}
& {\scriptsize \dots}     &{\scriptsize \dots} &{\scriptsize \dots} 	\\
%&&&&&&&&&\\
 {\scriptsize 07:09:30}  &{\scriptsize $4.69~~(0.04)$} &{\scriptsize $~~0.43~(0.04)$} &{~~~~}
& {\scriptsize 07:20:55}  &{\scriptsize $4.67~~(0.04)$} &{\scriptsize $~~0.93~(0.04)$} &{~~~~}
& {\scriptsize \dots}     &{\scriptsize \dots} &{\scriptsize \dots} 	\\
\hline
\hline
\end{tabular}
\end{center}
%\begin{list}{}{}
%\item[$n.d.$] Non Detection
%\end{list}


%\end{document}

